Aggregating explanation methods for stable and robust explainability

Despite a growing literature on explaining neural networks, no consensus has been reached on how to explain a neural network decision or how to evaluate an explanation. Our contributions in this paper are twofold. First, we investigate schemes to combine explanation methods and reduce model uncertainty to obtain a single aggregated explanation. We provide evidence that the aggregation is better at identifying important features, than on individual methods. Adversarial attacks on explanations is a recent active research topic. As our second contribution, we present evidence that aggregate explanations are much more robust to attacks than individual explanation methods.

==> tables/t_test_GradCAM.tex <==
\begin{tabular}{lrr}

        Evaluation method &  T statistic &   P-value \\
\midrule
           IROF (Black) &    4.73 &  3.23e-05 \\
IROF (Mean) &    7.81 &  2.42e-09 \\
Pixel flipping (Black) &   -1.75 &  8.85e-02 \\
Pixel flipping (Mean) &    3.26 &  2.38e-03 \\
Samek (2016) &    3.32 &  2.04e-03 \\
\end{tabular}


==> tables/t_test_GuidedBackprop.tex <==
\begin{tabular}{lrr}

        Evaluation method &  T statistic &   P-value \\
\midrule
           IROF (Black) &    3.79 &  5.42e-04 \\
IROF (Mean) &    5.64 &  1.93e-06 \\
Pixel flipping (Black) &    1.16 &  2.52e-01 \\
Pixel flipping (Mean) &    0.49 &  6.30e-01 \\
Samek (2016) &    3.02 &  4.54e-03 \\

\end{tabular}


==> tables/t_test_IGradients.tex <==
\begin{tabular}{lrr}
\toprule
        Evaluation method &  T statistic &   P-value \\
\midrule
  Segment flipping (Mean) &         7.19 &  3.32e-09 \\
    Pixel flipping (Mean) &         8.41 &  4.49e-11 \\
 Segment flipping (Black) &         2.85 &  6.42e-03 \\
   Pixel flipping (Black) &        -1.03 &  3.10e-01 \\
\bottomrule
\end{tabular}


==> tables/t_test_Saliency.tex <==

\begin{tabular}{lrr}

      Evaluation method &  T-stat &     P-val \\
\midrule
           IROF (Black) &    1.58 &  1.22e-01 \\
IROF (Mean) &    5.44 &  3.60e-06 \\
Pixel flipping (Black) &    1.92 &  6.22e-02 \\
Pixel flipping (Mean) &    2.10 &  4.25e-02 \\
Samek (2016) &    2.77 &  8.65e-03 \\
\end{tabular}

==> tables/t_test_SmoothGrad.tex <==
\begin{tabular}{lrr}

        Evaluation method &  T statistic &   P-value \\
\midrule
           IROF (Black) &    3.97 &  3.22e-04 \\
IROF (Mean) &    5.99 &  6.42e-07 \\
Pixel flipping (Black) &    0.55 &  5.86e-01 \\
Pixel flipping (Mean) &    5.00 &  1.39e-05 \\
Samek (2016) &    2.97 &  5.17e-03 \\
\end{tabular}

